Spherical formulation of geometric motion segmentation constraints in fisheye cameras

We introduce a visual motion segmentation method employing spherical geometry for fisheye cameras and automoated driving. Three commonly used geometric constraints in pin-hole imagery (the positive height, positive depth and epipolar constraints) are reformulated to spherical coordinates, making them invariant to specific camera configurations as long as the camera calibration is known. A fourth constraint, known as the anti-parallel constraint, is added to resolve motion-parallax ambiguity, to support the detection of moving objects undergoing parallel or near-parallel motion with respect to the host vehicle. A final constraint constraint is described, known as the spherical three-view constraint, is described though not employed in our proposed algorithm. Results are presented and analyzed that demonstrate that the proposal is an effective motion segmentation approach for direct employment on fisheye imagery.

==> algorithm.tex <==
\begin{algorithm}
 \caption{Estimating the motion likelihood (excluding three-view constraint)}
 \KwData{Set of correspondences $\left\{\mathbf{\acute{u}}_{i} \leftrightarrow \mathbf{\acute{u}'}_{i}\right\}$}
 \KwData{Rotation of camera against road surface $\mathbf{R}_{C}$}
 \KwData{Relative orientation $\mathbf{R}$ and translation $\mathbf{t}$}
 \KwResult{The set of motion likelihoods $\left\{\xi_i \right\}$ for each correspondence pair}
\begin{algorithmic}[1]
\FOR{all correspondence  $\left\{\mathbf{u}_{i} \leftrightarrow \mathbf{u}'_i\right\}$}
    \STATE Raise to rays on sphere $\left\{\mathbf{p}_{i} \leftrightarrow \mathbf{p}'_{i}\right\}$, per \S \ref{sec::Fisheye}
    
    \IF {$\mathbf{t} = \mathbf{0}$} 
        \STATE Calculate motion estimate $\xi$ using (\ref{eq:degen})
    \ELSE
        \STATE \COMMENT{Epipolar error}
        \STATE Get epipolar plane normal $\textbf{n}'$ per (\ref{eqn::epiPlane})
        \STATE Set $\xi_e$ according to (\ref{eqn::epiError})
        \STATE Project $\mathbf{p}'$ to the epipolar plane to get $\mathbf{p}'_\Pi$ by (\ref{eqn:posDepthProjEpi})
        \IF {$\mathbf{p}'$, $\mathbf{p}$ converge behind camera  (\ref{eqn:posDepthCross}) and (\ref{eq:posDepth})}
            \STATE Set positive depth error $\xi_d$ according to (\ref{eq:posDepth})
        \ELSE
            \STATE Set positive depth error $\xi_d = 0$
        \ENDIF
        \STATE Get horizon plane normal $\textbf{h}$ per (\ref{eq:horizon})
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> overview_table.tex <==
\begin{table*}[tbh]
\caption{Summary of the geometrical constraints used} 
\vspace{-0.5cm}
\label{table_1}
\begin{center}
\begin{tabular}{p{2cm} p{12cm} }
\hline
\multicolumn{2}{l}{\textbf{Planar epipolar constraint}}\\
\hline
Requires        & knowledge of camera ego-motion (scale not required)\\
Detected motion & crossing objects far from the epipolar plane \\
Limitations     & does not detect motion on the epipolar plane, which is common in road scenarios \\
\hline
\multicolumn{2}{l}{\textbf{Positive depth (cheirality) constraint}}\\
\hline
Requires        & knowledge of camera ego-motion (scale not required)\\
Detected motion & objects at higher speed than the ego-speed\\
Limitations     & does not help with detection of objects moving in the opposite direction \\
\hline
\multicolumn{2}{l}{\textbf{Positive height constraint}}\\
\hline
Requires        & knowledge of camera ego-motion (scale required) and rotation of the camera with respect to the road \\
Detected motion & preceding objects on the road with lower ego-speed \\
Limitations     & static points under the road plane level will be detected as moving as well (e.g. ground at a lower level beside the road, pot holes), applies only to points below the horizon line \\
\hline
\multicolumn{2}{l}{\textbf{Anti-parallel constraint}}\\
\hline
Requires        & knowledge of camera ego-motion (scale required) and rotation of the camera with respect to the road \\
Detected motion & approaching objects on the road with specular motion \\
Limitations     & static points above a determined height on the road plane level will be detected as moving as well, applies only to points below the horizon line \\
\hline
\multicolumn{2}{l}{\textbf{Three-view constraint}}\\
\hline
Requires        & knowledge of camera ego-motion (scale required (\textcolor{red}{tbd})), feature tracking over three frames \\
Detected motion & \textcolor{red}{tbd} \\
Limitations     & \textcolor{red}{tbd} \\
\hline
\end{tabular}
\end{center}
  \vspace{-0.6cm}
\end{table*}

